Monotonic Multihead Attention

Simultaneous machine translation models start generating a target sequence before they have encoded or read the source sequence. Recent approaches for this task either apply a fixed policy on a state-of-the art Transformer model, or a learnable monotonic attention on a weaker recurrent neural network-based structure. In this paper, we propose a new attention mechanism, Monotonic Multihead Attention (MMA), which extends the monotonic attention mechanism to multihead attention. We also introduce two novel and interpretable approaches for latency control that are specifically designed for multiple attentions heads. We apply MMA to the simultaneous machine translation task and demonstrate better latency-quality tradeoffs compared to MILk, the previous state-of-the-art approach. We also analyze how the latency controls affect the attention span and we motivate the introduction of our model by analyzing the effect of the number of decoder layers and heads on quality and latency.

==> sections/ablation.tex <==
\section{Analysis}

\subsection{Heads}

\begin{itemize}
    \item MMA enables us to use a state of the art model.
    \item Is there more to MMA?
    \item Ablation analysis: compare offline and online models for 1 dec layer and 1, 4, 8, 12, 16 heads and for 6 dec layers and 1, 4, 8, 12, 16 heads.
    TODO (fix those numbers, the configs are different for IWSLT and for WMT)
\end{itemize}

\subsection{Comparison with offline model on long sentences}

Idea: MMA is well suited for streaming, AKA long input.
We'd like to compare to MILk (which looks all the way to the beginning) but there's not much time to implement MILk on  RNMT+.
Instead we're going to compare to the offline model. Hopefully, we may get better results than the offline model similar to https://www.aclweb.org/anthology/P19-1290
